A Non-Iterative Algorithm for Clearing Two-Layer Energy-Sharing Markets with Voltage Constraints

Real-time hierarchical energy-sharing markets are promising to coordinate large numbers of prosumers. Still, most existing clearing methods rely on linearized or DC power-flow models and do not explicitly handle reactive power or voltage-security constraints. With AC network constraints, the problem becomes a large-scale bilevel Mathematical Program with Equilibrium Constraints (MPEC) that is difficult to solve in real time. This paper develops a non-iterative clearing algorithm for two-layer energy-sharing markets with voltage constraints. We first derive an efficient best-response function for each lower-layer energy-sharing market and reduce the equilibrium search to one dimension by exploiting the pricing-coupling structure. We then embed this function into the upper-layer network-constrained problem and reformulate the bilevel MPEC as a single-level mixed-integer second-order cone program (MISOCP), which is computationally tractable. Case studies on the IEEE 123-bus system with 12,300 prosumers show that the proposed method preserves nodal voltages within prescribed limits and delivers solutions with maximum errors below 0.01\% in 0.829 s.

==> old_closed_form.tex <==
Based on these fundamental dynamics, we first consider a scenario where prosumer parameters satisfy specific assumptions, leading to a closed-form solution.

\begin{assumption}\label{assump:closed_form}
    For all prosumers $m \in U_i$, $\beta_m \leq \gamma_m$ and $\max_{m \in U_i} \alpha_m < \min_{m \in U_i} \beta_m$.
\end{assumption}
\fliu{The rationality of the assumption should be clarified with justification.}

% 这别remark，说一下这玩意为啥基本正确
%不能够空口白牙，要么有数据，要么找文献
%文献的物理意义基本一致说明？
\begin{remark}
    Assumption \ref{assump:closed_form} physically implies sufficient generator capacity and relatively homogeneous cost coefficients among prosumers. These conditions are easily met in practice.
\end{remark}

% 闭式解可以挪掉
% 可以把remark放到算法后面

\begin{theorem}\label{theo:closed_form_X}
    Under Assumption \ref{assump:closed_form}, $X_i$ is a piecewise linear function of $w_i^0$ composed of $2n+1$ segments. Specifically, for segment index $j \in \{0, \dots, 2n\}$, $X_i$ satisfies:
    \begin{subequations}
    \begin{align}
        & \frac{w_i^--w_i^0}{a_i}n+(n+1)X_i = 0, \quad j=0 \label{eq:prop_j0} \\
        & \frac{w_i^--w_i^0}{a_i}(n-j) \notag \\
        & \quad + \sum_{s=1}^j \frac{w_i^--w_i^0 - c_{(s)}\alpha_{(s)}}{a_i+c_{(s)}} \notag \\
        & \quad + \left(n-j+1+\sum_{s=1}^{j}\frac{a_i}{a_i+c_{(s)}}\right)X_i = 0 \label{eq:prop_jmid} \\
        & \quad j=1,\dots,n-1 \notag \\
        & \sum_{s=1}^n\frac{c_{(s)}D_{(s)}+b_{(s)}-w_i^0}{c_{(s)}+a_i} \notag \\
        & \quad + \left(1+\sum_{s=1}^n\frac{a_i}{c_{(s)}+a_i}\right)X_i = 0, \quad j=n \label{eq:prop_jn} \\
        & \frac{w_i^+-w_i^0}{a_i}(j-n) \notag \\
        & \quad + \sum_{s=j-n+1}^{n} \frac{w_i^+-w_i^0 - c_{(s)}\beta_{(s)}}{a_i+c_{(s)}} \notag \\
        & \quad + \left(j-n+1+\sum_{s=j-n+1}^{n}\frac{a_i}{a_i+c_{(s)}}\right)X_i = 0 \label{eq:prop_jmid2} \\
        & \quad j=n+1,\dots,2n-1 \notag \\
        & \frac{w_i^+-w_i^0}{a_i}n+(n+1)X_i = 0, \quad j=2n \label{eq:prop_j2n}
    \end{align}
    \end{subequations}
    where $\alpha_{(s)}, \beta_{(s)}, c_{(s)}, D_{(s)}, b_{(s)}$ denote the parameters of the $s$-th prosumer sorted by the ascending order of $\alpha_m$.
\end{theorem}

The proof of Theorem \ref{theo:closed_form_X} is provided in Appendix \ref{app:E}.

\begin{theorem}\label{theo:closed_form_P}
    Under Assumption \ref{assump:closed_form}, $P_i$ is a piecewise linear function of $X_i$. Specifically, for segment index $j \in \{0, \dots, 2n\}$, $P_i$ satisfies:
    \begin{subequations}
    \begin{align}
        & P_i = \sum_{s=1}^n \alpha_{(s)}, \quad j=0 \label{eq:prop_P_j0} \\
        & P_i + \left(\sum_{s=1}^j \frac{a_i-k_{X,j}}{a_i+c_{(s)}}\right)X_i \notag \\
        & \quad = \sum_{s=1}^j \frac{b_{X,j} - b_{(s)} - c_{(s)} D_{(s)}}{a_i+c_{(s)}} \notag \\
        & \quad \quad + \sum_{s=j+1}^n \alpha_{(s)}, \quad j=1,\dots,n-1 \label{eq:prop_P_jmid} \\
        & P_i = X_i, \quad j=n \label{eq:prop_P_jn} \\
        & P_i + \left(\sum_{s=j-n+1}^n \frac{a_i-k_{X,j}}{a_i+c_{(s)}}\right)X_i \notag \\
        & \quad = \sum_{s=j-n+1}^n \frac{b_{X,j} - b_{(s)} - c_{(s)} D_{(s)}}{a_i+c_{(s)}} \notag \\
        & \quad \quad + \sum_{s=1}^{j-n} \beta_{(s)}, \quad j=n+1,\dots,2n-1 \label{eq:prop_P_jmid2} \\
        & P_i = \sum_{s=1}^n \beta_{(s)}, \quad j=2n \label{eq:prop_P_j2n}
    \end{align}
    \end{subequations}
    where $k_{X,j}$ and $b_{X,j}$ are the coefficients of the linear function $w_i^0 = k_{X,j}X_i + b_{X,j}$ obtained from the solution of the equations in Theorem \ref{theo:closed_form_X}.
\end{theorem}

The proof of Theorem \ref{theo:closed_form_P} is provided in Appendix \ref{app:C}.





    \section{Proof of Theorem \ref{theo:closed_form_X}}
    \label{app:E}
\begin{proof}
    Under Assumption \ref{assump:closed_form}, the migration path for all prosumers is Mode 3 $\to$ Mode 1 $\to$ Mode 2.
    Without loss of generality, assume prosumers are sorted such that $\alpha_{(1)} \le \alpha_{(2)} \le \dots \le \alpha_{(n)}$. 
    The segment index $j$ indicates the number of prosumers that have transitioned to the next mode.
    
    \textbf{Case 1: $j=0$.}
    All prosumers operate in Mode 3. Substituting the stationarity condition into $X_i = \sum_{s=1}^n x_{(s)}$ yields:
    \begin{equation}
        X_i = n \left( \frac{w_i^0 - w_i^-}{a_i} - X_i \right).
    \end{equation}
    Rearranging gives $\frac{w_i^--w_i^0}{a_i}n+(n+1)X_i = 0$, which matches \eqref{eq:prop_j0}.

    \textbf{Case 2: $j \in \{1, \dots, n-1\}$.}
    The first $j$ prosumers operate in Mode 1, and the remaining $n-j$ operate in Mode 3.
    Substituting their respective stationarity conditions into $X_i$:
    \begin{align}
        X_i &= \sum_{s=1}^j \frac{w_i^0 - b_{(s)} - c_{(s)} D_{(s)} - a_i X_i}{c_{(s)} + a_i} \notag \\
        &+ \sum_{s=j+1}^n \left( \frac{w_i^0 - w_i^-}{a_i} - X_i \right).
    \end{align}
    Rearranging to isolate $X_i$, we obtain:
    \begin{align}
        \left( n-j+1 + \sum_{s=1}^j \frac{a_i}{c_{(s)} + a_i} \right) X_i &= \sum_{s=1}^j \frac{w_i^0 - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i} \notag \\
        &+ \frac{w_i^0 - w_i^-}{a_i}(n-j).
    \end{align}
    Using $c_{(s)}\alpha_{(s)} = w_i^- - b_{(s)} - c_{(s)}D_{(s)}$, the equation becomes:
    \begin{align}
        \left( n-j+1 + \sum_{s=1}^j \frac{a_i}{c_{(s)} + a_i} \right) X_i &= \sum_{s=1}^j \frac{w_i^0 - w_i^- + c_{(s)}\alpha_{(s)}}{c_{(s)} + a_i} \notag \\
        &+ \frac{w_i^0 - w_i^-}{a_i}(n-j).
    \end{align}
    Moving all terms to the left yields the form in \eqref{eq:prop_jmid}.

    \textbf{Case 3: $j=n$.}
    All prosumers operate in Mode 1. Substituting the Mode 1 condition:
    \begin{align}
        \left( 1 + \sum_{s=1}^n \frac{a_i}{c_{(s)} + a_i} \right) X_i &= \sum_{s=1}^n \frac{w_i^0 - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i}.
    \end{align}
    This matches \eqref{eq:prop_jn}.

    \textbf{Case 4: $j \in \{n+1, \dots, 2n-1\}$.}
    The first $j-n$ prosumers operate in Mode 2, and the remaining $2n-j$ prosumers operate in Mode 1.
    Substituting their conditions:
    \begin{align}
        X_i &= \sum_{s=1}^{j-n} \left( \frac{w_i^0 - w_i^+}{a_i} - X_i \right) \notag \\
        &+ \sum_{s=j-n+1}^n \frac{w_i^0 - b_{(s)} - c_{(s)} D_{(s)} - a_i X_i}{c_{(s)} + a_i}.
    \end{align}
    Rearranging yields:
    \begin{align}
        \left( j-n+1 + \sum_{s=j-n+1}^n \frac{a_i}{c_{(s)} + a_i} \right) X_i=\notag \\
         (j-n)\frac{w_i^0 - w_i^+}{a_i} + \sum_{s=j-n+1}^n \frac{w_i^0 - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i}.
    \end{align}
    Using $c_{(s)}\beta_{(s)} = w_i^+ - b_{(s)} - c_{(s)}D_{(s)}$, we obtain the form in \eqref{eq:prop_jmid2}.

    \textbf{Case 5: $j=2n$.}
    All prosumers operate in Mode 2. Substituting the Mode 2 condition:
    \begin{equation}
        X_i = n \left( \frac{w_i^0 - w_i^+}{a_i} - X_i \right).
    \end{equation}
    Rearranging gives $\frac{w_i^+-w_i^0}{a_i}n+(n+1)X_i = 0$, which matches \eqref{eq:prop_j2n}.
    \end{proof}

\section{Proof of Theorem \ref{theo:closed_form_P}}
    \label{app:C}
    \begin{proof}
    From the definition of aggregate power exchange, $P_i = \sum_{m \in U_i} (x_m^* + p_m^{-*} - p_m^{+*})$.
    Based on Lemma \ref{lem:LSM_KKT}, the contribution of each prosumer depends on its operating mode:
    \begin{itemize}
        \item \textbf{Mode 1:} The contribution is $x_m$.
        \item \textbf{Mode 3:} The contribution is $\alpha_m$.
        \item \textbf{Mode 2:} The contribution is $\beta_m$.
    \end{itemize}
    
    From Theorem \ref{theo:closed_form_X}, the relationship between $X_i$ and $w_i^0$ is piecewise linear. 
    We define the linear function at segment $j$ as:
    \begin{equation}
        w_i^0 = k_{X,j} X_i + b_{X,j}.
    \end{equation}

    \textbf{Case 1: $j=0$.}
    All prosumers are in Mode 3.
    \begin{equation}
        P_i = \sum_{s=1}^n \alpha_{(s)}.
    \end{equation}
    This matches \eqref{eq:prop_P_j0}.

    \textbf{Case 2: $j \in \{1, \dots, n-1\}$.}
    Prosumers $s=1, \dots, j$ are in Mode 1, and $s=j+1, \dots, n$ are in Mode 3.
    \begin{equation}
        P_i = \sum_{s=1}^j x_{(s)} + \sum_{s=j+1}^n \alpha_{(s)}.
    \end{equation}
    From Lemma \ref{lem:LSM_KKT}, for Mode 1 prosumers:
    \begin{equation}
        x_{(s)} = \frac{w_i^0 - b_{(s)} - c_{(s)} D_{(s)} - a_i X_i}{c_{(s)} + a_i}.
    \end{equation}
    Substituting the linear relation $w_i^0 = k_{X,j} X_i + b_{X,j}$:
    \begin{equation}
        x_{(s)} = \frac{(k_{X,j} - a_i) X_i + b_{X,j} - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i}.
    \end{equation}
    Substituting this back into the expression for $P_i$:
    \begin{align}
        P_i &= \sum_{s=1}^j \frac{(k_{X,j} - a_i) X_i}{c_{(s)} + a_i} \notag \\
        &+ \sum_{s=1}^j \frac{b_{X,j} - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i} \notag \\
        &+ \sum_{s=j+1}^n \alpha_{(s)}.
    \end{align}
    Moving the summation involving $X_i$ to the left-hand side:
    \begin{align}
        P_i + \sum_{s=1}^j \frac{a_i - k_{X,j}}{c_{(s)} + a_i} X_i &= \sum_{s=1}^j \frac{b_{X,j} - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i} \notag \\
        &+ \sum_{s=j+1}^n \alpha_{(s)}.
    \end{align}
    This matches \eqref{eq:prop_P_jmid}.

    \textbf{Case 3: $j=n$.}
    All prosumers are in Mode 1.
    \begin{equation}
        P_i = X_i.
    \end{equation}
    This matches \eqref{eq:prop_P_jn}.

    \textbf{Case 4: $j \in \{n+1, \dots, 2n-1\}$.}
    Prosumers $s=1, \dots, j-n$ are in Mode 2, and $s=j-n+1, \dots, n$ are in Mode 1.
    \begin{equation}
        P_i = \sum_{s=j-n+1}^n x_{(s)} + \sum_{s=1}^{j-n} \beta_{(s)}.
    \end{equation}
    Following the same substitution logic as in Case 2:
    \begin{align}
        P_i + \sum_{s=j-n+1}^n \frac{a_i - k_{X,j}}{c_{(s)} + a_i} X_i &= \sum_{s=j-n+1}^n \frac{b_{X,j} - b_{(s)} - c_{(s)} D_{(s)}}{c_{(s)} + a_i} \notag \\
        &+ \sum_{s=1}^{j-n} \beta_{(s)}.
    \end{align}
    This matches \eqref{eq:prop_P_jmid2}.

    \textbf{Case 5: $j=2n$.}
    All prosumers are in Mode 2.
    \begin{equation}
        P_i = \sum_{s=1}^n \beta_{(s)}.
    \end{equation}
    This matches \eqref{eq:prop_P_j2n}.
    \end{proof}

==> old_draft.tex <==
\begin{abstract}
Ensuring voltage security in real-time energy sharing markets with a massive prosumer base is a critical yet computationally demanding task. Existing methods, when incorporating nonlinear AC power flow and voltage constraints, become computationally prohibitive for such large-scale applications. To address this issue, this paper proposes a non-iterative clearing algorithm for the two-layer hierarchical energy-sharing market. Our key innovation is deriving a closed-form best-response function for the lower-layer market, thereby transforming the complex bilevel Mathematical Program with Equilibrium Constraints (MPEC) into a tractable single-level mixed-integer second-order cone program (MISOCP). Case studies on systems with up to 33,000 prosumers validate our approach, demonstrating that the algorithm maintains all node voltages within secure limits while achieving a solution time of mere seconds. In contrast, benchmark methods exhibit prohibitive computation times. This work overcomes the critical trade-off between computational efficiency and voltage security, demonstrating the practical feasibility of real-time, large-scale, hierarchical energy markets.
\end{abstract}


\subsection{New Related Works}
Ensuring physical feasibility is the prerequisite for any viable energy sharing
market. Consequently, a significant line of research has focused on incorporating
network constraints, such as voltage limits and line capacities, into market
designs.To handle the non-convexity of AC power flow, the branch flow model
combined with Second-Order Cone Programming (SOCP) relaxation has become a
standard tool \cite{farivar_branch_2013}.
Concurrently,
pricing mechanisms like Distribution Locational Marginal Pricing (DLMP) and
decentralized market frameworks have been developed to mitigate congestion and
voltage violations \cite{golambahri_decentralized_2025}.Recent works have further expanded this domain to include transactive energy
trading and network-aware P2P frameworks\cite{yan_peer--peer_2023}.While these approaches
successfully address physical feasibility, they are predominantly limited to
single-layer or small-scale community markets, leaving the challenge of scaling
these rigorous models to massive systems largely unaddressed.

Scaling these market mechanisms to accommodate tens of thousands of prosumers
introduces severe computational challenges. Centralized optimization methods,
while robust, suffer from privacy concerns and the curse of dimensionality
in large-scale systems \cite{yaagoubi_energy_2017}.
Distributed algorithms,
particularly those based on the Alternating Direction Method of Multipliers
(ADMM), offer a promising alternative for coordination. However, the effectiveness
of distributed algorithms is highly sensitive to the complexity of physical
coupling. Research on ADMM-based optimal power flow in nested microgrids and
networked microgrid energy management indicates that enforcing the stringent
physical constraints mentioned earlier—specifically voltage and line
limits—severely degrades convergence performance \cite{noorpi_admm-based_2020,lou_span_2024,baek_security-constrained_2024,deng_parallel_2017,dong_dso-prosumers_2024}.The requirement for hundreds of iterations to
achieve consensus renders these pure distributed approaches impractical for
real-time clearing in physically constrained environments.

To bridge the conflict between the scalability of distributed architectures and the necessity of rigorous physical constraints, hierarchical or two-layer market frameworks have emerged. Approaches such as master-slave game scheduling and nested bilevel frameworks \cite{chen_two-layer_2024,lin_nested_2023,hong_bilevel_2023} attempt to retain rigorous physical constraints. However, these formulations typically result in complex Mathematical Programs with Equilibrium Constraints (MPEC) that require iterative solution processes, failing to meet the strict time constraints of real-time applications. Conversely, the seminal work by Su et al. \cite{su_sharing_2025} established a two-layer energy sharing scheme capable of accommodating over ten thousand prosumers. While this architecture successfully achieves scalability, it relies on a linearized power flow model, thereby overlooking the critical voltage security constraints required for physical feasibility.


Consequently, a critical research gap remains: no existing framework successfully integrates the scalability of two-layer architectures, the rigorous voltage security of physical constraints, and the computational efficiency of non-iterative clearing for massive, real-time applications. This gap stems from the lack of an efficient method to solve the single-period, high-dimensional, nonlinear Mathematical Program with Equilibrium Constraints (MPEC) that arise when integrating massive prosumers into an energy sharing market while explicitly considering nonlinear AC power flow and voltage security constraints.

\subsection{Related Works}
To tackle the core challenges of managing massive, self-interested, and 
variable prosumers while ensuring voltage security, the literature has 
explored several technical architectures for energy sharing. One line of research extends the traditional grid dispatch paradigm through 
centralized methods. These approaches typically require a central entity to 
gather comprehensive system information and solve a single, large-scale 
optimization problem to determine the dispatch for all prosumers. While 
capable of achieving a globally optimal solution, these methods face 
significant computational challenges with a large number of prosumers and 
may not align with the autonomous nature of participants 
\cite{udabala_aggregated_2025,ivanov_flexible_2024}.

As an alternative, distributed methods have been widely investigated, 
ranging from optimization algorithms like the Alternating Direction 
Method of Multipliers (ADMM) 
\cite{soto_peer--peer_2021,baek_security-constrained_2024} 
to decentralized market-based trading platforms 
\cite{guerrero_decentralized_2019}.
These approaches allow prosumers to reach a global consensus, 
offering enhanced scalability iteratively. However, their convergence performance can 
be sensitive to the number of participants \cite{deng_parallel_2017}. 
More importantly, the convergence rate may be significantly slowed when 
essential network security constraints, such as the nonlinear AC power 
flow equations are incorporated. For instance, the work in 
\cite{dong_dso-prosumers_2024} reported convergence times on the order 
of hundreds of seconds for a network with only 8 prosumers when the voltage 
constraints were considered, highlighting a significant computational 
bottleneck for real-time, large-scale applications.

To reconcile the advantages of centralized coordination for system-wide 
constraints with the scalability of distributed optimization, the hierarchical distributed market framework has emerged as a promising 
direction \cite{su_sharing_2024}. This architecture typically consists of an Upper-Layer Energy Sharing Market (U-ESM) that coordinates multiple Lower-Layer Energy Sharing Markets (L-ESMs), aligning well with the 
hierarchical management of distribution networks and enabling wider-area 
energy trading. The pioneering work in \cite{su_sharing_2024} established 
such a foundational two-layer framework using a linear power flow model, 
successfully demonstrating its potential.

However, extending this framework to address the complexities of nonlinear 
AC power flow and its associated voltage security constraints remain an 
open and critical research question. Therefore, a clear research gap 
remains in the state-of-the-art: the lack of an efficient method to solve 
the single-period, high-dimensional, nonlinear Mathematical Program with 
Equilibrium Constraints (MPEC) that arise when integrating massive 
prosumers into an energy sharing market while explicitly considering 
nonlinear AC power flow and voltage security constraints within a 
hierarchical framework.

So the preliminary mathematical model is as follows:
\begin{subequations}\label{model:simple_stage_raw}
    \begin{align}
    &\min_{w_i^0,P_i,Q_i,P_{ij},Q_{ij},l_{ij},v_i} \sum_{(i,j)\in \mathcal{E}} r_{ij}l_{ij} \label{obj:USM}\\
    \text{s.t.} \notag\\
    &P_j = \sum_{k:j \to k} P_{jk} - \sum_{i:i \to j} (P_{ij} - r_{ij}l_{ij}), \forall j \in \mathcal{N} \label{cons:node_P} \\
    &Q_j = \sum_{k:j \to k} Q_{jk} - \sum_{i:i \to j} (Q_{ij} - x_{ij}l_{ij}), \forall j \in \mathcal{N} \label{cons:node_Q}\\
    &v_j = v_i - 2(r_{ij}P_{ij}+x_{ij}Q_{ij})
    + (r^2_{ij} + x^2_{ij})l_{ij} \label{cons:node_v} \\
    &\phantom{v_j = v_i - 2(r_{ij}P_{ij}+x_{ij}Q_{ij}) + (r^2_{ij} + x^2_{ij})l_{ij}} \makebox[0pt][r]{\ensuremath{\forall (i,j) \in \mathcal{E}}} \notag \\
    &P_{ij}^2 + Q_{ij}^2 = l_{ij}v_{i},\forall (i,j) \in \mathcal{E} \label{cons:line_limit}\\
    &\underline{v_i} \leq v_i \leq \overline{v_i},\forall i \in \mathcal{N}\label{cons:v_lb_ub}\\
    &0 \leq l_{ij} \leq \overline{l_{ij}},\forall (i,j) \in \mathcal{E} \label{cons:l_lb_ub}\\
    &P_j = \sum_{m \in U_j}(x^*_m+p_m^{-*}-p_m^{+*}),\forall j \in \mathcal{N}\label{cons:P_define}\\
    &X_j = \sum_{m \in U_j}x^*_m,\forall j \in \mathcal{N}\label{cons:X_define}\\
    &\sum_{i \in \mathcal{N}}X_i = 0\label{cons:sum_X}\\
    &w_i = w_i^0 - a_iX_i,\forall i \in \mathcal{N}\label{cons:supply_demand}\\
    &s_m^* = \{p_m^*,p_m^{+*},p_m^{-*},x_m^*\}, \forall m \in U_i,\forall i \in \mathcal{E} \notag\\
    &\quad =\arg \min_{p_m,p_m^+,p_m^-,x_m}\frac{c_m}{2}p_m^2+b_mp_m+w^+_ip_m^+\notag\\
    &\phantom{\quad =\arg \min_{p_m,p_m^+,p_m^-,x_m}\frac{c_m}{2}p_m^2+b_mp_m+w^+_ip_m^+} \makebox[0pt][r]{\ensuremath{-w_i^-p_m^--w_ix_m}} \label{obj:LSM_raw}\\
    &\text{s.t.} \notag\\
    &\qquad D'_m +x_m+p^-_m = p_{solar,m}+p_m + p_m^+ \label{cons:energy_balence_raw}\\
    &\phantom{\qquad D'_m +x_m+p^-_m = p_{solar,m}+p_m + p_m^+} \makebox[0pt][r]{\ensuremath{\forall m \in U_i}}\notag \\
    &\qquad 0 \leq p_m \leq \overline{p_m},\forall m \in U_i \label{cons:p_lb_ub}\\
    &\qquad p_m^+ \geq 0,p_m^- \geq 0,\forall m \in U_i \label{cons:p_+_-}\\
    &\qquad p_m^+p_m^- = 0,\forall m \in U_i \label{cons:su_relax}
    \end{align}
\end{subequations}






where $\mathcal{E}$ is the branch set of a power system,
$r_{ij},x_{ij},l_{ij},P_{ij},Q_{ij}$ represent the impedance, inductive reactance, 
square of the current, active power, and reactive power of the corresponding branch, respectively.
$P_i,Q_i,v_i$ represent the injected active power, reactive power, and voltage at node $i$, respectively.
For a particular prosumer $m$, $x_m$ is its shared energy. 
$x_m > 0$ if prosumer $m$ is a seller,while $x_m < 0$ if prosumer $m$ is a buyer.
$p_m,D^{'}_m,p_{solar,m}$ denote the adjustable power generation,
the load and the non-adjustable power generation of prosumer $m$.
$p_m^+$ and $p_m^-$ denotes the purchased and sold electricity from/to the electric utility.
$c_m > 0$ and $0 < b_m<w_i^-$ are constant parameters of the adjustable power generator cost.
For a particular L-ESM $i$,$w_i$ denotes the energy sharing price,
while $w_i^0$ is the base price controlled by the L-ESM operator and $a_i >0$ is the price elasticity.
We define the market uncleared sharing energy $X_i = \sum_{m \in U_i} x_m$ 
and the actual node power $P_i = \sum_{m \in U_i}x_m +p_m^--p_m^+$.

\begin{subequations}\label{model:simple_stage}
    \begin{align}
    &\min_{w_i^0,P_i,Q_i,P_{ij},Q_{ij},l_{ij},v_i} \eqref{obj:USM} \notag\\
    \text{s.t.} \notag\\
    &\labelcref{cons:node_P,cons:node_Q,cons:node_v,cons:line_limit,cons:v_lb_ub,cons:l_lb_ub,cons:P_define,cons:X_define,cons:sum_X}
    \notag\\
    s_m^* &= \{p_m^*,p_m^{+*},p_m^{-*},x_m^*\}\forall m \in U_i,\forall i \in \mathcal{E} \notag\\
    &= \arg \min_{p_m,p_m^+,p_m^-,x_m}
    \sum_{m \in U_i} (\frac{c_m}{2}p_m^2+b_mp_m+w^+_ip_m^+ \notag\\
    &\phantom{= \arg \min_{p_m,p_m^+,p_m^-,x_m}
    \sum_{m \in U_i} (\frac{c_m}{2}p_m^2+b_mp_m+w^+_ip_m^+} \makebox[0pt][r]{\ensuremath{\displaystyle -w_i^-p_m^--w_i^0x_m)+\frac{a_i}{2}(\sum_{m \in U_i}x_m^2) + \frac{a_i}{2}(\sum_{m \in U_i}x_m)^2}} \\
    &\text{s.t.} \notag\\
    &\qquad\labelcref{cons:p_lb_ub,cons:p_+_-}\notag\\
    &\qquad D_m +x_m+p^-_m = p_m + p_m^+,\forall m \in U_i
    \end{align}
\end{subequations}

\begin{lemma}\label{lem:LSM_KKT}
    For the prosumer component $\{p_m^*,p_m^{+*},p_m^{-*},x_m^*\}$ of 
    the optimal solution to the optimization problem \eqref{model:L-ESM subproblem},
    one of the following conditions must be satisfied:
    \begin{enumerate}
        \item $c_m(x_m^*+D_m)+b_m-w_i^0+a_i(x_m^*+x_{-m}^*)+ a_ix_m^* = 0$,$p_m^* = x_m^*+D_m$
        \item $w_i^+-w_i^0 + a_i(x_m^*+x_{-m}^*) + a_ix_m^* = 0$,$p_m^* = \min(\overline{p_m},\frac{w_i^+-b_m}{c_m})$
        \item $w_i^--w_i^0 + a_i(x_m^*+x_{-m}^*) + a_ix_m^* = 0$,$p_m^* = \min(\overline{p_m},\frac{w_i^--b_m}{c_m})$
        \item $x_m^* = \overline{p_m} - D_m$,$p_m^* = \overline{p_m}$
    \end{enumerate}
where, $x_{-m}^* := \sum_{j \in U_i, j\neq m}x_j^* ,\forall m \in U_i.$
\end{lemma}
The proof of lemma \ref{lem:LSM_KKT} can be found in Appendix \ref{app:A}.

\begin{proof}
    Applying the KKT conditions yields:
    \begin{equation}\label{dL_d}
        \begin{aligned}
        c_mp_m+b_m-\lambda_{eq,m}-\lambda_{p,lb,m}+\lambda_{p,ub,m} = 0\\
        w_i^+-\lambda_{eq,m}-\lambda_{p,+,m} = 0\\
        -w_i^-+\lambda_{eq,m}-\lambda_{p,-,m} = 0\\
        -w_i^0+a_ix_m+a_i(x_m+x_{-m})+\lambda_{eq,m} = 0
        \end{aligned}
    \end{equation}
    Next,discuss by cases $p_+ = 0 \land p_- = 0$,$p_+ \neq 0 \land p_- = 0$,
    $p_- \neq 0 \land p_+ = 0$.

    Under case $p_+ = 0 \land p_- = 0$,formula \eqref{dL_d} can be simplified to:
    \begin{equation*}
        \begin{aligned}
        c_mp_m+b_m-\lambda_{eq,m}= 0\\
        w_i^+-\lambda_{eq,m}-\lambda_{p,+,m} = 0\\
        -w_i^-+\lambda_{eq,m}-\lambda_{p,-,m} = 0\\
        -w_i^0+a_ix_m+a_i(x_m+x_{-m})+\lambda_{eq,m} = 0
        \end{aligned}
    \end{equation*}
    And we can get $D_m + x_m = p_m$.

    If $p_m = \overline{p_m}$,the condition 4 is satisfied.

    If $p_m < \overline{p_m}$,we can obtain by rearranging:
    \begin{align*}
        c_mp_m+b_m-w_i^0+a_ix_m+a_i(x_m+x_{-m}) = 0 \\
        = c_m(x_m+D_m)+b_m-w_i^0+a_ix_m+a_i(x_m+x_{-m})
    \end{align*}
    then the condition 1 is satisfied.

    Other cases can be analyzed similarly.
    \end{proof}

\begin{lemma}\label{lem:P_with_X}
    $P_i(w_i^0)$ and $X_i(w_i^0)$ both are piecewise linear functions and every breakpoint of $P_i(w_i^0)$ is necessarily a breakpoint of $X_i(w_i^0)$.
\end{lemma}

\begin{proof}
    According to lemma \ref{lem:LSM_KKT}, either $p_m^* = x_m^*+D_m$ or $p_m^*$ is a constant.
    Meanwhile $P_i(w_i^0)$ and $X_i(w_i^0)$ undergo mode changes simultaneously.
\end{proof}

\begin{lemma}\label{lem:dx_dw_i^0}
    The shared energy of a specific prosumer $x^*_m$and the uncleared sharing energy of an LSM $X_i$ are both non-decreasing in the base price $w_i^0$.
    \begin{equation*}
        \frac{\mathrm{d} x^*_m}{\mathrm{d} w_i^0} \geq 0 ,\forall m \in U_i;\qquad \frac{\mathrm{d} X_i}{\mathrm{d} w_i^0} \geq 0
    \end{equation*}
\end{lemma}

\begin{proof}
    Consider differentiating both sides of the equations satisfied by 
    the prosumer components of the optimal solution in lemma \ref{lem:LSM_KKT} 
    with respect to $w_i^0$,This yields:
    \begin{enumerate}
        \item $(c_m+a_i) \frac{\mathrm{d} x^*_m}{\mathrm{d} w_i^0}-1 + a_i \frac{\mathrm{d} (x^*_m+x^*_{-m})}{\mathrm{d} w_i^0} = 0,\forall m \in U_{i1}$
        \item $a_i \frac{\mathrm{d} x^*_m}{\mathrm{d} w_i^0}-1 + a_i \frac{\mathrm{d} (x^*_m+x^*_{-m})}{\mathrm{d} w_i^0} = 0,\forall m \in U_{i2}$
        \item $\frac{\mathrm{d} x^*_m}{\mathrm{d} w_i^0} = 0,\forall m \in U_{i3}$
    \end{enumerate}
    where $U_i = U_{i1} \bigsqcup U_{i2} \bigsqcup U_{i3}$.
    Denote $$\frac{\mathrm{d} x^*_m}{\mathrm{d} w_i^0} = x^{'}_m,
    \frac{\mathrm{d} x^*_{-m}}{\mathrm{d} w_i^0} = x^{'}_{-m},x^{'}_m+x^{'}_{-m} = x^{'}_{\Sigma}$$
    We obtain:
    \begin{enumerate}
        \item $(c_m+a_i)x^{'}_m + a_ix^{'}_{\Sigma} = 1,\forall m \in U_{i1}$
        \item $a_ix^{'}_m + a_ix^{'}_{\Sigma} = 1,\forall m \in U_{i2}$
        \item $x^{'}_m = 0,\forall m \in U_{i3}$
    \end{enumerate}
    By appropriate summation, we derive:
        \begin{align*}
        &\sum_{m \in U_{i1}}(x^{'}_m+\frac{a_i}{c_m+a_i}x^{'}_{\Sigma})
        +\sum_{m \in U_{i2}}(x^{'}_m+x^{'}_{\Sigma})
        +\sum_{m \in U_{i3}}(x^{'}_m)\\
        =&\sum_{m \in U_{i1}}(\frac{1}{c_m+a_i})
        +\sum_{m \in U_{i2}}(\frac{1}{a_i})
        +\sum_{m \in U_{i3}}(0)
    \end{align*}
    \begin{equation*}
        (1+\sum_{m \in U_{i1}}\frac{a_i}{c_m+a_i}+\sum_{m \in U_{i2}}1)x^{'}_{\Sigma}=
        \sum_{m \in U_{i1}}(\frac{1}{c_m+a_i})+\sum_{m \in U_{i2}}(\frac{1}{a_i})
    \end{equation*}
    Since $c_m>0,a_i>0$, $x^{'}_{\Sigma} \geq 0$

    Additionally, consider:
    \begin{align*}
        (\frac{1}{a_i}+\sum_{m \in U_{i1}}\frac{1}{c_m+a_i}+\sum_{m \in U_{i2}}\frac{1}{a_i})a_ix^{'}_{\Sigma}=\\
        \sum_{m \in U_{i1}}(\frac{1}{c_m+a_i})+\sum_{m \in U_{i2}}(\frac{1}{a_i})
    \end{align*}

    So:
    \begin{align*}
        a_ix^{'}_{\Sigma} < 1\\
        -1+a_ix^{'}_{\Sigma} < 0\\
        x^{'}_m \geq 0
    \end{align*}
\end{proof}


It is noted that in the optimization model \eqref{model:simple_stage}, 
$w_i^0$ exclusively affects the $X_i$ and $P_i$ of the L-ESM $i$ subproblem,
which in turn participate in other constraints.
A natural approach is to completely replace the L-ESM subproblem 
with $X_i(w_i^0)$ and $P_i(w_i^0)$. 
According to lemma \ref{lem:dx_dw_i^0} and \ref{lem:piecewise}, 
$X_i$ is monotonically increasing in $w_i^0$.
Therefore,a further approach is to directly replace L-ESM subproblem with $P_i(X_i)$
and change the decision variables of the optimization problem \eqref{model:simple_stage}
to $X_i$,namely, resulting in the following optimization problem:


\begin{subequations}\label{model:simple_stage_with_X}
    \begin{align}
    &\min_{X_i,P_i,Q_i,P_{ij},Q_{ij},l_{ij},v_i} \eqref{obj:USM} \notag\\
    \text{s.t.} \notag\\
    &P_j(X_j)  = \sum_{k:j \to k} P_{jk} - \sum_{i:i \to j} (P_{ij} - r_{ij}l_{ij}), \forall j \in \mathcal{N} \label{cons:P_node_new}\\
    &\labelcref{cons:node_Q,cons:node_v,cons:v_lb_ub,cons:l_lb_ub,cons:sum_X}\notag\\
    &P_{ij}^2 + Q_{ij}^2 \leq l_{ij}v_{i},\forall (i,j) \in \mathcal{E} \label{cons:line_limit_relaxed}\\
    &\underline{X_i} \leq X_i \leq \overline{X_i},\forall i \in \mathcal{N}\label{cons:X_lb_ub}
    \end{align}
\end{subequations}

    \begin{proof}
    If the constraints are not tight,it implies that for the optimal solution of problem \eqref{model:simple_stage_with_X}$\{X_i^*,P_i^*,Q_i^*,P_{ij}^*,Q_{ij}^*,l_{ij}^*,v_i^*\}$,$$P_{i^{'}j^{'}}^{*2} + Q_{i^{'}j^{'}}^{*2} < l_{i^{'}j^{'}}^*v_{i^{'}}^*,\exists (i^{'},j^{'}) \in \mathcal{E}$$.
    Consider the following optimization problem:
    \begin{equation*}
    \begin{aligned}
&\min_{P_i,Q_i,P_{ij},Q_{ij},l_{ij},v_i} \sum_{(i,j)\in \mathcal{E}} r_{ij}l_{ij}\\
    s.t. P_j  &= \sum_{k:j \to k} P_{jk} - \sum_{i:i \to j} (P_{ij} - r_{ij}l_{ij}), \forall j \in \mathcal{N}\\
    Q_j  &= \sum_{k:j \to k} Q_{jk} - \sum_{i:i \to j} (Q_{ij} - x_{ij}l_{ij}), \forall j \in \mathcal{N}\\
    v_j - v_i&=  - 2(r_{ij}P_{ij}+x_{ij}Q_{ij}) + (r^2_{ij} + x^2_{ij})l_{ij},\forall (i,j) \in \mathcal{E}\\
    P_{ij}^2 + Q_{ij}^2 &\leq l_{ij}v_{i},\forall (i,j) \in \mathcal{E}\\
    \underline{v_i} &\leq v_i \leq \overline{v_i},\forall i \in \mathcal{N}\\
    0 &\leq l_{ij} \leq \overline{l_{ij}},\forall (i,j) \in \mathcal{E}\\
   P_i^*  &\leq P_i \leq P_i^*,\forall i \in \mathcal{N}
    \end{aligned}
\end{equation*}

which should share the same optimal solution $\{P_i^*,Q_i^*,P_{ij}^*,Q_{ij}^*,l_{ij}^*,v_i^*\}$.
Then the inactive constraint $P_{i^{'}j^{'}}^{*2} + Q_{i^{'}j^{'}}^{*2} < l_{i^{'}j^{'}}^*v_{i^{'}}^*$ contradicts Theorem 1 of Paper \cite{farivar_branch_2013},therefore the proposition holds.  
% 这里可能要检查一下定理使用条件
\end{proof}




Since we already know that $X_i(w_i^0)$ and $P_i(X_i)$ are 
piecewise functions,a piecewise analysis is warranted.

\begin{lemma}\label{lem:the_leftest}
    When 
    \begin{equation*}
        \frac{w_i^0-w_i^-}{a_i(1+n)}\leq \min \{\min_{m \in U_i}(\frac{w_i^--b_m}{c_m}-D_m),\min_{m \in U_i}(\overline{p_m}-D_m) \}
    \end{equation*}
    we have
    \begin{equation*}
        x_m^* = \frac{w_i^0-w_i^-}{a_i(1+n)},\forall m \in U_i;X_i = \frac{w_i^0-w_i^-}{a_i}\frac{n}{1+n}
    \end{equation*}
    where $n = |U_i|$     
\end{lemma}
% 如果引入一些符号，这里可以变得简洁一点。

\begin{proof}
    According to lemma \ref{lem:LSM_KKT},under given condition,all prosumers are in mode 3,
    so we summarize them and get:
    $$
    n(w_i^--w_i^0)+na_iX_i+a_iX_i = 0
    $$
    and then we can get $X_i$ and condition for the lemma to hold,further get $x_m^*$.
\end{proof}

We denote the breakpoints of $X_i(w_i^0)$ as $BP_i,i \in N$.
According to lemma \ref{lem:initial_segment},$BP_0 = -\infty,BP_1 = w_i^-+a_i(1+n)min_{m \in U_i}(\frac{w_i^--b_m}{c_m}-D_m)$.
If we can sequentially generate the next piece of the piecewise function, then we can recursively obtain the entire function.

When $BP_i \leq w_i^0 \leq BP_{i+1}$,depending on how 
each prosumer satisfies Lemma \ref{lem:LSM_KKT}'s condition, 
partitioning can be performed accordingly.
$U_i = U_{i1} \bigsqcup U_{i2} \bigsqcup U_{i3} \bigsqcup U_{i4}$.
Once a prosumer moves from one set to another,it introduces a
breakpoint to the piecewise function.
Based on the preceding discussion, there are exclusively 
three possible paths for prosumer migration: 
Path $U_{i3}\to U_{i1}\to U_{i2}$,Path $U_{i3}\to U_{i4}\to U_{i2}$and 
Path $U_{i3}\to U_{i1}\to U_{i4}\to U_{i2}$. 
All prosumers initially reside in Set $U_{i3}$ and
ultimately transition to Set $U_{i2}$.

% 这里要不要说明那个所有人处在U_{i4}然后死住的情况呢，这需要很极端且凑巧的参数
% 要说，仿真的时候会出现

According to lemma \ref{lem:LSM_KKT} and \ref{lem:dx_dw_i^0},we can further 
derive the conditions for prosumer migration between these sets:

\begin{lemma}\label{lem:prosumer_move}
    If $\overline{p_m}>\frac{w_i^+-b_m}{c_m}$,prosumer $m$ moves along Path $U_{i3}\to U_{i1}\to U_{i2}$;
    If $\overline{p_m}\leq\frac{w_i^--b_m}{c_m}$,prosumer $m$ moves along Path $U_{i3}\to U_{i4}\to U_{i2}$;
    Otherwise,prosumer $m$ moves along Path $U_{i3}\to U_{i1}\to U_{i4}\to U_{i2}$.
    The conditions for prosumer migration are as follows:
    \begin{enumerate}
        \item $U_{i3}\to U_{i1}:p_m^*-D_m = x_m^* = \frac{w_i^--b_m}{c_m}-D_m$
        \item $U_{i3}\to U_{i4}:p_m^* = \overline{p_m} = x_m^*+D_m$
        \item $U_{i1}\to U_{i4}:p_m^* = \overline{p_m} = x_m^*+D_m$ 
        \item $U_{i1}\to U_{i2}:p_m^*-D_m = x_m^* = \frac{w_i^+-b_m}{c_m}-D_m$
        \item $U_{i4}\to U_{i2}:X_i = \frac{w_i^0-w_i^+}{a_i}-x_m^* = \frac{w_i^0-w_i^+}{a_i}-\overline{p_m}+D_m$
    \end{enumerate} 
\end{lemma}

% 这里补一个proof

\begin{remark}
    \label{re:X_i(w_i^0)}
    While the above algorithm applies to all parameters, more direct results can be obtained under certain easily satisfied assumptions.
    
    If we have $\beta_m \leq \gamma_m,\forall m \in U_i$ and $\max(\alpha_m)<\min(\beta_m)$,then the $X_i$ and $w_i^0$ satisfy:
    \begin{align*}
        \frac{w_i^--w_i^0}{a_i}n+(n+1)X_i = 0,j=0\\
        \frac{w_i^--w_i^0}{a_i}(n-j)+\sum_{s=1}^j\frac{w_i^--w_i^0}{a_i+c_s}+\sum_{s=1}^{j}\frac{-c_s\alpha_s}{a_i+c_s}\\+(n-j+1+\sum_{s=1}^{j}\frac{a_i}{a_i+c_s})X_i = 0,\\j=1,2\cdots,n-1\\
        \sum_s\frac{c_sD_s+b_s-w_i^0}{c_s+a_i}+(1+\sum_s\frac{a_i}{c_s+a_i})X_i = 0,j=n\\
        \frac{w_i^+-w_i^0}{a_i}(j-n)+\sum_{s=j-n+1}^{n}\frac{w_i^+-w_i^0}{a_i+c_s}+\sum_{s=j-n+1}^{n}\frac{-c_s\beta_s}{a_i+c_s}\\+(j-n+1+\sum_{s=j-n+1}^{n}\frac{a_i}{a_i+c_s})X_i = 0,\\j=n+1,n+2\cdots,2n-1\\
        \frac{w_i^+-w_i^0}{a_i}n+(n+1)X_i = 0,j=2n
    \end{align*}
    which is readily computable using only $\alpha_m$ and $\beta_m$ obtained from each prosumer since $c_m = \frac{w_i^+-w_i^-}{\beta_m-\alpha_m}$.
    %说一下交点分界
    
    Notably,these conditions are not difficult to achieve.
    The physical meaning of condition $\beta_m \leq \gamma_m$ is
    that the upper bound of prosumers' generator is not too small,while condition $\max(\alpha_m)<\min(\beta_m)$ implies
    that the cost coefficients of the generators among different prosumers do not vary significantly.These are conditions the prosumers can easily meet.
\end{remark}

\begin{remark}
    Under the same conditions as in Remark \eqref{re:X_i(w_i^0)},$P_i(X_i)$ can also be empressed in closed form:
    \begin{align*}
        P_i &= \sum_{s=1}^n\alpha_s,j=0\\
        P_i &+ (\sum_{s=1}^j\frac{a_i-k_{X,j}'}{a_i+c_s})X_i+\sum_{s=1}^j\frac{b_s-b_{X,j}'-a_iD_s}{a_i+c_s} = \sum_{s=j+1}^n\alpha_s\\&j=1,2\cdots,n-1\\
        P_i &= X_i,j = n\\
        P_i &+ (\sum_{s=j-n+1}^n\frac{a_i-k_{X,j}'}{a_i+c_s})X_i+\sum_{s=j-n+1}^n\frac{b_s-b_{X,j}'-a_iD_s}{a_i+c_s}\\
        &= \sum_{s=1}^{j-n}\beta_s \qquad
        j=n+1,n+2\cdots,2n-1\\
        P_i &= \sum_{s=1}^n\beta_s,j=2n
    \end{align*}
    where $k_{X,j}' = \frac{1}{k_{X,j}},b_{X,j}' = \frac{-b_{X,j}}{k_{X,j}}$,$k_{X,j},b_{X,j}$are the coefficients for the corresponding piece of function $X_j(w_i^0)$
\end{remark}

Subsequently,an intuitive algorithm for calculating $X_i(w_i^0)$ can be derived.

\begin{algorithm}
    \caption{Computation of $X_i(w_i^0)$}
    \label{alg:X_i(w_i^0)}
    \KwIn{$w_i^+$,$w_i^-$,$a_i$,$n:=|U_i|$,$\alpha_m:=\frac{w_i^--b_m}{c_m}-D_m$,$\beta_m:=\frac{w_i^+-b_m}{c_m}-D_m$,$\gamma_m:=\overline{p_m}-D_m$}
    \KwOut{$X_i(w_i^0),State_{idx,m}$}

    $BP_0 = -\infty$\;
    $idx = 1$\;
    $State_{idx,m} = 3,\forall m\in U_i$\;
    \While{true}{
        \For{$m \in U_i$}{
            \tcp{Based on $State_{idx,m}$ and Lemma \eqref{lem:LSM_KKT}}
            Obtain the equations satisfied by each prosumer\;
            }
        Obtain the equation satisfied by $X_i$ through accumulation\;
        Update $k_{X,idx},b_{X,idx}$\;
        \tcp{Based on Lemma \eqref{lem:prosumer_move}}
        Calculate the $w_{i,idx,m}^0$ that each prosumer needs to move to the next state\;
%state的名词统一性也许需要处理一下，各个位置好像用的英文不太一样
        $BP_{idx} = \min_{m}(w_{i,idx,m}^0)$\;
        Update $State_{idx+1,m}$ of the corresponding prosumer.\;
        $idx = idx +1$\;
        \If{$BP_{idx} = +\infty$}{
            break\;
        }
    }
    Assemble $X_i(w_i^0)$ using $k_{X,idx},b_{X,idx}$
\end{algorithm}



Following the computation of $X_i(w_i^0)$,$P_i(X_i)$can be subsequently determined based on the $X_i(w_i^0)$ and information obtained in the process.

According to the lemma \ref{lem:LSM_KKT}, for a particular prosumer $m \in U_i$,$p_m^*$ equals $x_m^*+D_m$ or is a constant, depending on the set in which the prosumer is located.So an algorithm can be derived to calculate $P_i(X_i)$.

\begin{algorithm}
    \caption{Computation of $P_i(X_i)$}
    \label{alg:P_i(X_i)}
    \KwIn{$State_{idx,m},X_i(w_i^0),\alpha_m,\beta_m,\gamma_m,D_m,a_i,n$}
    \KwOut{$P_i(X_i)$}
    \For{$idx = 1,2,\cdots$}{
        \For{$m \in U_i$}{
            \tcp{Based on $State_{idx,m}$ and Lemma \eqref{lem:LSM_KKT}}
            Obtain the equations satisfied by each prosumer\;
            Eliminate $w_i^0$ from the equations
            }
        Obtain this piece of $P_i(X_i)$ by accumulation.
    }
    Assemble the whole $P_i(X_i)$
\end{algorithm}


\subsection{Verification of Voltage Constraints}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{image_case_v.png}
    \caption{Enter Caption}
    \label{fig:placeholder}
\end{figure}



The case33bw network is utilized for this experiment. The number of prosumers in each L-ESM is set to 100, which amounts to a total of 3300 prosumers. Energy sharing is conducted separately with method\cite{su_sharing_2025} and our proposed method. The voltage situation across the entire network obtained from these methods is presented in the figure below:




It can be observed that the voltages from the proposed method all remain within the required voltage limits, while  method\cite{su_sharing_2025} leads to numerous voltage violations.


%In contrast, benchmark methods exhibit prohibitive computation times. 
%This work overcomes the critical trade-off between computational efficiency and voltage security guarantee, demonstrating the practical feasibility of real-time, large-scale, hierarchical energy markets.

%Existing mechanisms often struggle to reconcile the conflicting requirements of computational efficiency, economic optimality, and physical security, particularly in scenarios involving tens of thousands of participants and strict voltage regulations. 

%Scaling these market mechanisms to accommodate tens of thousands of prosumers introduces severe computational challenges. Centralized optimization methods, while capable of achieving globally optimal solutions, suffer from privacy concerns and the curse of dimensionality in large-scale systems \cite{udabalaAggregatedEnergyInteraction2025}. Distributed algorithms, ranging from game-theoretic approaches \cite{yaagoubiEnergyTradingSmart2017} to decentralized market-based trading platforms \cite{sotoPeertopeerEnergyTrading2021, guerreroDecentralizedP2PEnergy2019}, offer a promising alternative for coordination. In particular, the Alternating Direction Method of Multipliers (ADMM) has gained significant traction due to its ability to decompose large-scale optimization problems. However, the effectiveness of distributed algorithms is highly sensitive to the complexity of physical coupling. Research on ADMM-based optimal power flow and voltage control indicates that enforcing stringent physical constraints severely degrades convergence performance \cite{noorpiADMMbasedOptimumPower2020, louADMMBasedDistributed2024, baekSecurityConstrainedP2PEnergy2024, dengParallelMultiBlockADMM2017, liuDistributedVoltageControl2018, fengPeertoPeerEnergyTrading2023}. For instance, the work in \cite{dongDSOprosumersDuallayerGame2024} reported convergence times on the order of tens of seconds for a network with only 8 prosumers when voltage constraints were considered, highlighting a significant computational bottleneck for real-time, large-scale applications.

%It is noted that in the optimization model \eqref{model:simple_stage}, the base price $w_i^0$ influences the U-ESM solely through the aggregate variables $X_i$ and $P_i$ of the L-ESM subproblem. According to Lemmas \ref{lem:piecewise} and \ref{lem:dx_dw_i^0}, the function $X_i(w_i^0)$ is piecewise linear and non-decreasing. Crucially, this monotonicity ensures that for any given $X_i$, the corresponding $P_i$ is uniquely determined, even in the extreme case (Mode 4) where $X_i$ is constant with respect to $w_i^0$. This property allows us to reformulate the problem by replacing the implicit L-ESM equilibrium constraints with the explicit best-response function $P_i(X_i)$ and choosing $X_i$ as the decision variable. Consequently, the original bilevel model \eqref{model:simple_stage} can be transformed into the following single-level optimization problem:


%Ensuring physical feasibility, such as voltage security, is crucial for any viable energy sharing market. Consequently, a significant line of research has focused on incorporating network constraints, such as voltage limits and line capacities, into market designs. To handle the non-convexity of AC power flow, the branch flow model combined with Second-Order Cone Programming (SOCP) relaxation has become a standard tool cite{farivarBranchFlowModel2013}. Concurrently, pricing mechanisms like Distribution Locational Marginal Pricing (DLMP) and decentralized market frameworks have been developed to mitigate congestion and voltage violations \cite{golambahriDecentralizedEnergyFlexibility2025, wuOptimalManagementTransactive2020}. Recent works have further expanded this domain to include transactive energy trading and network-aware P2P frameworks \cite{yanPeertoPeerTransactiveEnergy2023, yanDistributionNetworkConstrainedOptimization2021}. Additionally, the coordination of shared resources such as energy storage has been explored to enhance system flexibility \cite{yanDistributedCoordinationCharging2023}. While these approaches successfully address physical feasibility, they are predominantly limited to single-layer or small-scale community markets, leaving the challenge of scaling these rigorous models to massive systems largely unaddressed.
